Query By Provenance

To assist non-specialists in formulating database queries, multiple frameworks that automatically infer queries from a set of examples have been proposed. While highly useful, a shortcoming of the approach is that if users can only provide a small set of examples, many inherently different queries may qualify, and only some of these actually match the user intentions. Our main observation is that if users further explain their examples, the set of qualifying queries may be significantly more focused. We develop a novel framework where users explain example tuples by choosing input tuples that are intuitively the "cause" for their examples. Their explanations are automatically "compiled" into a formal model for explanations, based on previously developed models of data provenance. Then, our novel algorithms infer conjunctive queries from the examples and their explanations. We prove the computational efficiency of the algorithms and favorable properties of inferred queries. We have further implemented our solution in a system prototype with an interface that assists users in formulating explanations in an intuitive way. Our experimental results, including a user study as well as experiments using the TPC-H benchmark, indicate the effectiveness of our solution.

==> lin.tex <==
\section{Additional Semirings}
\label{sec:more}

So far we have considered the case where full derivations (but
perhaps not all) are given ($\NX$), and the case where the use of
the same tuple multiple times in a derivation is masked (Trio).
Explaining tuples through the notion of derivations, with every
derivation corresponding to an alternative explanation, is very
natural in cases such as the one of our running example -- where
each explanation is a desired trip. However, there are cases where
the technical notion of derivation does not have such interpretation
that is clear to the non-expert. In these cases, it would be easier
for users to ``explain" an output tuple by detailing a set of
relevant input tuples -- i.e. to provide the tuple {\em lineage}
\cite{lin} as an explanation.

\begin{example}
\daniel{TBD: exemplify}
\end{example}


%Trying to learn a query from lineage, we face a new challenge of


Interestingly, the freedom in ``breaking" the set of annotations
into monomials allows to show an even better bound for the ``small
world" property, compared to the one shown for Trio:

\begin{proposition}
\label{prop:triobound} For any {\lin} example, if there exists a
consistent query then there exists a consistent query with $k+r$
atoms or less, where $r$ is the number of relations in $D^{in}$.
\end{proposition}


\begin{proof}
\daniel{TBD}
\end{proof}


\IncMargin{1em}
\begin{algorithm}
    \SetKwFunction{LinAlgo}{ComputeQueryLin}
    \SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
    \LinesNumbered
    \Input{A Lin example Ex}
    \Output{A consistent query $q$ or an answer that none exists} \BlankLine

    Treat each lineage expression as a single monomial to obtain $\{(t_0,M_0),...,(t_n,M_n)\}$ \;
    $Q \gets (t_0,M_0)$ \;
    \ForEach{$1 \leq i\leq n$} {
     $(V,E) \gets BuildGraph((t_i,M_i),Q)$ \;
     $match \gets false$ \;
     \ForEach {{\em sub-graph} $E' \subseteq E \text{ s.t. } |E'| \leq k \text{~~and~~} \cup_{e \in E'} label(e) = \{1, \ldots, k\}$}
     {
       $match \gets true$ \;

       \ForEach{conjunct $C \in Q$}
       {
        Let $t'_1,...,t'_p$ be the tuples whose annotations are
        connected by edges in $E'$ to $C$ \;
        $Q \gets Q \cup split(C) - \{C\}$ \;
       }

       \ForEach{{\em relation name} $R$ of a tuple corresponding to an annotation in $M_i$ that is not an end point of an edge in $E'$}
       {
         $Q \gets Q \cup NewAtom(R)$ \;
        }
       }
    \If{$match = false$}
    {
    Continue and try next query \;
    }
    }
    \If{a match was found in all steps}
    {
    return $Q$ \;
    }

    Output ``No consistent query exists"\;





\caption{FindConsistentQuery (Lin)}\label{algo:lin}
\end{algorithm} \DecMargin{1em}



Similarly to the case of trio, we may use the bound to consider all
options of $\NX$ provenance expressions that are consistent with the
given lineage. Again similarly to the case of trio, we can do much
better if we gradually consider the different options based on the
matchings we obtain. Algorithm \ref{algo:lin} is similar to
Algorithm \ref{algo:trio}, with subtle differences that we next
highlight. We start by considering the set of annotations comprising
the lineage of each tuple, as if they are all members of a single
monomial. We then proceed as in the trio algorithm, but the main
difference is that we only generate as many atoms as needed to cover
the head, without worrying about covering additional provenance
annotations. The observation is that to use all remaining provenance
atoms it suffices to add a single atom per relation name from which
these annotations were taken. This atom is assigned fresh variables,
so that it may match any tuple of the relation.

\daniel{Not exactly $1$, what if we have multiple relation names}
\paragraph*{Complexity} Since the generated query size is bounded by $k+r$, the complexity is again $O(m^O(k+r) \cdot n)$.


\begin{example}
\daniel{TBD:example}
\end{example}


\paragraph*{Discussion} \daniel{If we keep like that, discuss the disadvantages of obtained queries. One idea: disqualify queries that are not minimal in the standard sense.}


==> minimization.tex <==
\section{Choosing Best Candidates}
\label{sec:minimization}

\subsection{Query Optimization: Standard Minimization versus p-minimization}

\subsection{Most tight fit}


==> results.tex <==
\section{Results and Main Algorithm Ideas}

\daniel{More for ourselves, I think the gist of it will have to go
to the Intro}


\subsection{\NX}


==> userStudy.tex <==
\subsection{User Study}
\label{sec:userstudy}
We have examined the usefulness of the system to non-expert users. To this end, we have loaded the IMDB database to \systemName\ (see a partial schema in Figure \ref{scehma}) and have presented each of the tasks in Table \ref{tasks} to 15 users. We have also allowed them to freely choose tasks of the likings, resulting in a total of 120 performed tasks. The intended queries are presented in Table \ref{queries}, where the relation {\em atm} stands for ActorsToMovies.        

% The experiment then consisted of two steps: first, we have asked users to perform the tasks in Table \ref{tasks} by providing the system with examples and explanations; then we have allowed users to choose questions of their liking, and again interact with the system to have these questions answered. The study consisted of 15 participants \amir{cur. have 13}, where each was asked to perform 7 tasks, combining to a total of 105 system interactions. In addition, we allowed the users to come up with their own tasks. 




%
%In this study, we aimed to understand the feasibility of a non-expert user providing output examples and explanations for the system.
%For the user study, we have used \systemName\ as described in Section \ref{sec:imp} with the IMDB dataset \cite{imdb}. The user tasks are shown in Table \ref{tasks}.  

%\paragraph*{Study Settings}


%To give an example, the user would copy the output value/values from the table (e.g., copy the actor name from the actor table) and drag the tuples he think were needed to explain why he chose this value (e.g., the tuple that states that the actor played in Pulp Fiction). All intended queries consist of five atoms or less. 
%similar to the sample given in Figure \ref{fig:imdb}
%Once the user has finished with the examples, he would press on the ``Find Query'' button which would allow the system to find the query using the aforementioned algorithms and evaluate it using IRIS \cite{iris}.

\begin{figure}[]
	\begin{center}
		\includegraphics[trim = 0mm 0mm 0mm 0mm, clip = true, width=3in]{IMDB_Schema_cropped}
		\vspace{-2mm} \caption{Partial IMDB schema} \vspace{-3mm}
		\label{scehma}
	\end{center}
\end{figure}


\begin{table}[!htb]
	\centering \scriptsize
	\begin{tabular}{l | p{7.7cm} }
		\hline & {\bf Task} \\ 
		\hline
		1. & Find all actresses \\
		2. & Find all movies that came out in 1994 \\
		3. & Find all of Al Pacino's movies \\
		4. & Find the entire cast of Pulp Fiction \\
		5. & Find all documentary films (by having character ``Himself'') \\
		%6. & Find pairs of actors who played in two movies together \\
		6. & Find the actors who played in all the 3 movies of The Lord Of The Rings \\
		7. & Choose an actor and two movies he played in, and find all actors that played with him in these two movies \\
		%
		%Instead of 4: 9. Choose an actor and two movies he played in, and
		%find all actors that played with him in these two movies.
		%
		%Sometimes give the example and sometimes not. Maybe analyze what
		%would have happended without the explanation.
		%
		%Did they succeed, and how difficult was it?
		
		\hline
	\end{tabular}
	\caption{User Tasks}\label{tasks}
	\vspace{-2mm}
\end{table}

%Order of questions in Iris Experiment. Do not delete!
%\begin{table}[!htb]
%    \centering
%    \begin{tabular}{l  l }
%        \hline & {\bf Task} \\
%        \hline
%        1. & Find all actresses \\
%        2. & Find all of Al Pacino's movies \\
%        3. & Find the entire cast of Pulp Fiction \\
%        %4. & Find the actors who played both in Pulp Fiction and in Reservoir Dogs \\
%        5. & Find pairs of actors who played in two movies together \\
%        6. & Find all movies that came out in 1994 \\
%        7. & Find the actors who played in all the 3 movies of Jurassic Park \\
%        8. & Find all documentary films (by character) \\
%        9. & Choose an actor and two movies he played in, and find all actors that played with him in these two movies \\
%%
%%Instead of 4: 9. Choose an actor and two movies he played in, and
%%find all actors that played with him in these two movies.
%%
%%Sometimes give the example and sometimes not. Maybe analyze what
%%would have happended without the explanation.
%%
%%Did they succeed, and how difficult was it?
%
%        \hline
%    \end{tabular}
%    \caption{User Tasks}\label{tasks}
%\end{table}


\begin{table}[!htb]
	\centering \scriptsize
	\begin{tabular}{l |  p{7.7cm} }
		\hline & {\bf Queries} \\ 
		\hline 
		1. & ans(t) :- actors(mid, t, 'F') \\
		2. & ans(t) :- movies(mid, t, '1994') \\ %actorsToMovies
		3. & ans(t) :- atm(mid, aid, c), actors(aid, 'Pacino, Al', 'M'), movies(mid, t, y) \\
		4. & ans(n) :- atm(mid, aid, c), movies(mid, 'Pulp Fiction', '1994'), actors(aid, n, s) \\
		5. & ans(t) :- atm(mid, aid, 'Himself'), actors(aid, n, 'M'), movies(mid, t, y) \\
		6. & ans(n) :- atm(mid1, aid, c), atm(mid2, aid, c), atm(mid3, aid, c), actors(aid, n, s), movies(mid1, 'The Fellowship of the Ring', '2001'), movies(mid2, 'The Two Towers', '2002'), movies(mid3, 'The Return of the King', '2003') \\
		\hline
	\end{tabular}
	\caption{Queries (No. 7 depends on user choices, omitted)}\label{queries}
	\vspace{-4mm}
\end{table}


%Overall the vast majority of users (80\%) were successful in properly formulating examples and explanations for all tasks.

In 111 out of the 120 cases, including all cases of freely chosen tasks, users were successful in specifying examples and explanations, and the interface of \systemName\ was highly helpful in that.  



\begin{example}
%\daniel{We need an example that illustrates all parts: how the system's proposals helped users in formulating explanations, what were the examples and the explanations, how was the query inferred and what would happen if not. Build upon the following. }
Consider task 6 in Table \ref{tasks}. The examples are actor names; for every chosen actor name, \systemName\ has proposed as explanations only the tuples that included this actor name as one of its values.  In particular, the tuples of  $ActorsToMovies$ corresponding to movies in which the actor has played were proposed. Knowing the underlying task, it was natural for users to choose the relevant movies, namely the three ``Lord Of The Rings" movies. Once they did that, the tuples of these movies (and not of any other movie) in the $Movies$ relation has appeared as proposals, allowing their easy selection. A similar case is that of task 3: once a movie is specified as an example, the system proposes its actors as possible explanations. The choice of Al Pacino as an explanation reveals the underlying intention.  
\end{example}


%Consider task 3 in Table \ref{tasks}, and consider the very partial schema in Figure \ref{scehma}. Examples here are movie titles; for every specified movie title (say, ``The godfather"), \systemName\ has proposed as explanations only the tuples that included ``The godfather" as one of its values. In particular, the tuples of  ``ActorsToMovies" corresponding to ``The godfather" actors were proposed. This has naturally led the users to choose the fact that Al Pachino is an actor in the Godfather as explanation; then the ``Al Pachino" tuple in the Actors relation is further proposed, leading to a completion of the explanation.   


%These include the tuples of.      
%
%
%note that without explanations, there is little chance that the   
%
%In task 3, users were asked to provide examples of Al Pcino's movies and explanations that say Al Pacino acted in this movie. Users gave movie titles as outputs (A popular example was ``The Godfather'' movies) and their desired explanations included the movie tuple (out of the ``Movies" table), the Al Pacino tuple (out of the ``Actors" table) and the tuple that connected the movie to Al Pacino (out of the ``ActorsToMovies" table). 
%
%When users chose the movie title as output, the system showed only the tuples that have the same constants as the movie tuple, i.e., the movie tuple itself and the ``ActorsToMovies"  tuples that have the same m\_id as the m\_id of the movie (e.g., for ``The Godfather", the system showed only the tuples of actors who played in ``The Godfather" in the ``ActorsToMovies" table). Intuitively, the system allowed the user to decide if he chose the movie because of its properties or because of an actor/character in the movie.
%Users then chose the explanation to be the tuple from the ``ActorsToMovies'' table that relates to both Al Pacino and the movie given as an output example (e.g., the tuple (The Godfather id, Al Pacino id, Michael Corleone)). Once this tuple was added to the explanation, the Al Pacino tuple in the ``Actors" table appeared. Intuitively, now the Al Pacino tuple is also relevant as it relates to the previously chosen tuple, so it may help explain it.


%Since this feature removed almost all tuples from the tables, it made the task of finding explanations much easier, and indeed all users succeeded in giving the right tuple as an explanation. 


%In one case, a user wrote the movie id as an output example instead of the movie name, which caused the system to output the wrong query. 

%\amir{go over next part} Two main features of the system were used here; the filter option was used by users who did not recall Al Pacino's work and the auto-completion of an explanation i.e., completing the explanation to consist of the ``ActorsToMovies'' tuple the user gave and the corresponding ``Actors'' and ``Movies'' tuples (based on actor id and movie id).
	
In turn, explanations were crucial for allowing the system to focus on the intended query, even with very few examples (in all cases users provided at most 4 examples). 

\begin{example}
	
	%\amir{add more examples from mail and explain in detail}
	
	Re-consider task 6, and now assume that explanations are unavailable. There would be no way of distinguishing the underlying query from, for instance, a much simpler one that looks for the actors of a {\em single} Lord of the rings. More generally, join conditions (or even the fact that a join took place) are in many cases only apparent through the explanations: another example is task 3, where examples are simply movie names that typically have many other characteristics in common in addition to having Al Pacino acting in them. In addition to revealing join conditions, explanations help to learn the query constants: for instance, in task 4, without explanations, the resulting query could have returned all actors who played in a movie with Quentin Tarantino.
	   
	%unless this explanation was provided, the system could infer a different query, e.g., a query that returns all movies who have male actors in them. 
\end{example}


Out of the 9 cases where users failed to provide examples and explanations, 5 involved difficulties in providing any example matching the task, and 4 involved errors in providing explanations. Out of the remaining 111 cases, in 98 cases \systemName\ has inferred the actual underlying query, and in the remaining 13 cases, it has inferred a ``more specific" query (i.e. with extra constants). This for instance happened when all actors given as examples were males. We next further analyze the accuracy of \systemName.  

%Despite the overall high success rates, we have observed some difficulties of several kinds:
%
%\begin{enumerate} 
%\item In the pre-defined tasks 4 and 6, 5 \amir{in one or the other} users had difficulties coming up with any examples, and eventually had to resort to a search engine for examples. Naturally, this did not happen in the part of the experiments where users could freely choose examples. Moreover, while the need for users to be able to provide examples is a feature of any example-based system, it is much less of a limitation here, since 2--3 examples typically sufficed for the system to converge to the correct result. 
%\item In the pre-defined task 6, one user got confused when specifying the explanations. Namely, he gave three examples; one of an actor name explained by the fact he played in the first movie, one of an actor who played in the second movie and one from the third. This was an exception to the general rule of users specifying sound explanations.    
%\end{enumerate} 
%
%The resulting query was of course always consistent with the given examples and explanations. For task 4 and for 27\% of the users, the derived query was more specific, i.e. included additional constants, than the one specified in the task. This was the case when only very few (2--3) examples were given and both the examples and the explanations had a shared constant ``by coincidence". For instance, some users initially provided only examples of male actors, in which case an extra corresponding constant has appeared in the inferred query. See further discussion of this phenomenon in the following subsection.
%   
%
%
%
%%The first and second tasks are simple projection queries and require an actress (movie) name as an output example and one atom from the ``actors'' (``movies'') table as an explanation. Users used the filter field in the GUI to find the actors whose sex is ``Female'' and the movies whose year is ``1994'' and gave two of the result as examples. Due to the help of filtering, all users were able to find two correct output examples and explanations for both tasks. Any two examples of actresses in the first task and movies in the second, were sufficient for the system to output the correct query (see Table \ref{queries}). Users did not need directions on how to give examples and explanations for this task and the tasks seemed intuitive to them.
%%
%%Task number 3 presented the more illusive challenge of understanding what the output should be and mainly, what is the explanation (notice that this is the first query that requires a join operation). Outputs were movie names (A popular example was ``The Godfather'' movies) and the explanation was a tuple from the ``actorsToMovies'' table that relates to both Al Pacino and the movie given as an output example (e.g., the tuple (The Godfather id, Al Pacino id, Michael Corleone)). In one case, a user wrote the movie id as an example instead of the movie name, which caused the system to output the wrong query. Two main features of the system were used here; the filter option was used by users who did not recall Al Pacino's work and the auto-completion of an explanation i.e., completing the explanation to consist of the ``actorsToMovies'' tuple the user gave and the corresponding ``actors'' and ``movies'' tuples (based on actor id and movie id).
%%
%%In the fourth task, users were asked to find the entire cast of the movie ``Pulp Fiction'', which also translates to a join query in IMDB. In the terms of our experiment, they were asked to understand they have to give two or more examples of actor names who played in ``Pulp Fiction'' as outputs and explain each name with the corresponding ``actorsToMovies'' tuple that forms the connection between the actor and the movie ``Pulp Fiction''. John Travolta, Uma Thurman and Steve Buscemi were popular examples for this task and the system returned the correct query in all attempts. A common issue here was giving two examples of male (female) actors (actresses) which caused the system to infer the query that returns all male (female) actors  (actresses) that played in ``Pulp Fiction''. In addition, the users did not require help in giving the examples and explanations for this task. As in the previous example, users used the filter and explanation auto-completion for the convenience of giving examples.
%% 
%%Next, users were asked to find all documentary films, not by genre but by character (also resulting in a join query). In the ``actorsToMovies'' table, the character field may have the value ``Himself'' or ``Herself'', hence the users had to give examples of movie names and explain them with tuple from the ``actorsToMovies'' table which relate the name of the movie they chose to the character name ``Himself'' or ``Herself''. One user accidentally gave the actor names instead of the movie names as the output examples, resulting in a query that finds all actors who played in documentary films. Another user gave one example with the character ``Himself'' and the other example with the character ``Herself''. The system did not recognize that both characters suggest documentary films, so it found a query that returns all films. Beside these cases, the users were able to formulate examples and explanations for this task as well and the system outputted the intended query.   
%%
%%In Task 6, users needed to find examples of actors who played in all 3 ``Lord of The Rings'' movies and explain each choice of actor with the 3 corresponding ``actorsToMovies'' tuples that makes the connection between the chosen actor and the first, second and third movies. For example, the 3 tuples that form an explanation for the output ``Liv Tyler'' are (The Fellowship of The Ring id, Liv Tyler id, Arwen), (The Two Towers id, Liv Tyler id, Arwen) and (The Return of The King id, Liv Tyler id, Arwen). Here, even when using the filter, users who did not know the series of movies had a though time finding examples of actors, so sometimes, a web search was needed. All users gave 2 examples and once the examples were given, the system found the intended query.
%%
%%Task 7 is more fluid in the sense that it does not direct the user to a specific movie of actor but rather allows the user to select the actor she is interested in and then find two movies she was a part of. Users who completed this task (which can be done solely with the filter option) needed to find the actors who played in the two movies together. Popular pairs here were ``Reservoir Dogs'' and ``The Lord of The Rings'' again, while for the actors, users chose ``Quentin Tarantino'' and ``Orlando Bloom''. As in the previous task, some users needed to search the web for the second example. 
%%%for the query that will produce all actors who played in these two movies together.   
%%
%%
%%Finally, users were asked to try a query of their own and see if the results are what they had in mind. Users usually tried variations of the tasks given to them like ``find all actresses who played in the Lord of The Rings trilogy'' and ``Find all men actors in documentary films''. Since the users came up with the query themselves and they had gained some experience with the system thus far, they did not need help in finding examples and explanations for this task and were able to assemble the input for the system, composed of 2 examples. The system was able to find the intended query in all cases.
%%
%%Users were also asked about \systemName's ease of use on a scale of 1-5. The average result was 2.5.
%%
%%\paragraph*{Insights}
%%The study gave us several important insights into the usability of the system. A simple problem encountered by a large portion of the users is the difficulty in the variety of constants in the explanation tuples. For instance, when the users tried to find the cast of ``Pulp Fiction'', they gave two examples of male actors, which caused the system to infer a query that returns all the {\em male} actors who played ``Pulp Fiction''. Furthermore, as the explanation required more tuples, the users had a tougher time understanding what tuples to include in the explanations and how should the explanation be structured. E.g., In task 6, a user gave an example where the output was an actor and the explanation was that he played in the first movie, another example where the output was an actor and the explanation was that he played in the second movie and the same for the third movie. The output was correct but the explanation should have been that the actor played in all three movies, i.e., three tuples for each explanation. In addition, in several of the harder tasks, the users struggled to find examples for outputs, e.g., task 4 was hard for people who did not watch ``Pulp Fiction''. On the other hand, in task 7, when the users were asked to come up with their own queries, it was much easier for them to find examples.
%%
%%
%%\paragraph*{Study Conclusions}
%%To conclude, the user study allowed us to determine that the system is usable for non-expert users. The most significant findings is that sometimes users will have a challenge producing examples for the system and give explanations tuples with sufficiently varied constants, especially if the intended query is a complex join query. However, when the tasks are not dictated and the users can decide what to ask, they can often produce examples for the query they have in mind. Furthermore, we have observed that for all tasks, 2--3 examples were sufficient for the system to produce the intended query.    
%%
%%
%%
%%%In all cases, the users reported that two examples were sufficient for satisfactory results and the inferred queries matched the expected queries. With regards to the ease-of-use, users claimed it was less intuitive that the explanation should contain the answer itself, i.e., that the head variables should also appear in the body. However, other than this issue, the non-expert users reported no considerable effort in providing a couple of explanations and were content with the results.
%%
%%
%%
%%
%%  
%%%For every question I will do the experiment. If I didn't find the query, explain why (e.g., did not have examples to give). If successful, how many examples. If not, why not? (Avarage time, maybe?). Second part: choose your own questions after all the questions given have been answered 
%%
%%%Amir: Questions 1-3, 6 are easy for the user since they usually involve one explanation tuple and do not require a join operation. The system learns the intended query with two examples. The challange with questions 4 and 7 is finding examples. Once examples are given by the user (using Google, for example), the system learns a more general query from two examples (bug) i.e. in question 4, the query is correct but the constants 'Pulp Fiction' and 'Reservoir Dogs' do not appear. In question 8, the challange is to understand what is a good example and explanation. The output tuple should be the name of the movie and the explanation should be the an actorsToMovies tuple with the character field being 'Himself'. Here the system finds the intended query with two good examples.  
%%%
%%%Iris: easy to use and write the explanations and all queries were consistent with my expectations after a single try consisting of two examples
%%
%%Amit and Brit: quite hard to understand that the output of the query should appear in the explanations but after understanding that, it is quite easy to use and the output matched my expectations
%%
%%Yuval:
%%
%%Ahmad:
%%
%%Amir:
%%
%%Slava:
%%
%%Ofer:
%%
%%Alon:

